Efficient Schedulability Test for Dynamic-Priority Scheduling of Mixed-Criticality Real-Time Systems

Systems in many safety-critical application domains are subject to certification requirements. In such a system, there are typically different applications providing functionalities that have varying degrees of criticality. Consequently, the certification requirements for functionalities at these different criticality levels are also varying, with very high levels of assurance required for a highly critical functionality, whereas relatively low levels of assurance required for a less critical functionality. Considering the timing assurance given to various applications in the form of guaranteed budgets within deadlines, a theory of real-time scheduling for such multi-criticality systems has been under development in the recent past. In particular, an algorithm called Earliest Deadline First with Virtual Deadlines (EDF-VD) has shown a lot of promise for systems with two criticality levels, especially in terms of practical performance demonstrated through experiment results. In this paper we design a new schedulability test for EDF-VD that extend these performance benefits to multi-criticality systems. We propose a new test based on demand bound functions and also present a novel virtual deadline assignment strategy. Through extensive experiments we show that the proposed technique significantly outperforms existing strategies for a variety of generic real-time systems.

==> Technique_1.tex <==

\section{Improved Single-Mode DBF (ISM) Based Test For MC Task Systems}
\label{sec:GIO}
The dbf summarized in Section~\ref{sec:ExistDBF} and  presented in ~\cite{EkYi12,EkYi14}  is pessimistic in the sense that it would over estimate the demand of carry-over jobs.  We  use a simple example in Figure~\ref{fig:dbfc4} to illustrate this shortcoming.
\begin{example}
As shown in Figure~\ref{fig:dbfc4}, consider carry-over jobs $J_1^m$ and $J_2^m$, where $d(J_1^m,m-1)=r(J_1^m)+D_i^{m-1}=4$ and $d(J_2^m,m-1)=r(J_2^m)+D_2^{m-1}=4$. $J_1^m$ is supposed to generate $3$ time units demand during the time interval $[0,4]$, while $J_2^m$ is supposed to generate $3$ time units demand during the time interval $[0,3]$ if the system does not switch to $L_m$ mode.  This implies that there exists at least two time units during which $J_1^m$ and $J_2^m$ execute simultaneously if mode-switch does not happen, and this is impossible on an uniprocessor platform.

Assuming no deadline miss happens in $L_{m-1}$ criticality mode, the demand generated in the time interval $[0,4]$ cannot be greater than $4$ (otherwise deadline miss happens in $L_{m-1}$ criticality mode). Thus in this  release  pattern,  there exists at least $2$ time units of  over-estimated execution demand that should be already finished by $S_m$.
\label{example:e1}
\end{example}

% %=================================================================================================
\begin{figure}[tbh]
\begin{center}
\noindent
  \includegraphics[scale=0.8]{fig/dbfc4}
  \end{center}
  \caption{Overestimated Demand of Carry-Over Jobs}
\label{fig:dbfc4}
\end{figure}
% %=================================================================================================

From Section~\ref{sec:ExistDBF}  we know $\tau_i$ generates maximum demand in $L_m$ criticality mode for time interval $[S_m, S_m+\mathit e]$ with the release pattern in Lemma~\ref{lemma:pt1}: the  virtual deadline  of the last job $J_i^{L}$ released before $\mathit e$ is at $S_m+\mathit e$, i.e., $d(J_i^L,m)=r(J_i^L)+D_i^m=\mathit e$. Therefore we can easily  identify the scheduling window of the carry-over job $J_i^m$ of $\tau_i$, and compute the remaining demand of $J_i^m$ during $[S_m, d(J_i^m,m-1)]$ Let $RMD_i^m$ denote the maximum possible remaining demand of a carry-over job $J_i^m$ at $S_m$, that should be finished by $d(J_i^m,m-1)$ if the system does not switch to $L_m$ mode.   
\begin{equation}
\label{eqn:dbffi}
\begin{split}
RMD_i^m=
   \begin{cases}
 C_i^{m-1}-done_m(\tau_i,\mathit e)&  \mbox{If } mod(\mathit e,T_i)-D_i^m+D_i^{m-1}\geq 0\\
0& \mbox{otherwise}
    \end{cases}
\end{split}
\end{equation}
where $done_m(\tau_i,\mathit e)$  is given in Equation~\ref{eqn:done}.

% \footnote{Later in Lemma~\ref{propostion:proposition1} we prove that the total execution demand maximizes when all tasks are released with such pattern in Lemma~\ref{lemma:pt1}.}. 
\begin{figure}[th]
\centering
  \includegraphics[scale=0.8]{fig/dbfc5}
\caption{Remove Overestimated Demand}
\label{fig:dbfc5}
\end{figure}

Consider the set of jobs $J^m = \{ J_i^m | RMD_i^m > 0 \}$, and without loss of generality let us assume that these job indices are sorted in deadline order. That is, $\forall i$ and $j$ with $j>i$  s.t. $J_i^m$ and $J_j^m \in J^m$:  $d(J_i^m,m-1)\leq d(J_{j}^m,m-1)$. As shown in Figure~\ref{fig:dbfc5}, $J_1^m$ can generate $RMD_1^m$ demand during $\left[S_m,~d(J_1^m,m-1)\right)$.  Let  $AS_1^m$ denote the available time slots for $J_1^m$  to execute remaining execution demand $RMD_1^m$.  $AS_1^m$ is equal to $d(J_1^m,m-1)$.
Carry-over job  $J_2^m$ is supposed to generate $RMD_2^m$ demand during $\left[S_m,~S_m+d(J_2^m,m-1)\right)$ while the available time slots for it to finish this demand is $AS_2^m=d(J_2^m,m-1)-d(J_1^m,m-1)+(d(J_1^m,m-1)-RMD_1^m)$, because $J_1^m$ has already occupied $RMD_1^m$ time units.  Since the available time slots  for $J_2^m$,  $AS_2^m$, is smaller than $RMD_2^m$, it implies that $J_2^m$ must have  finished at least $OD_2(m)=RMD_2^m-AS_2^m$ execution demand before $S_m$. Therefore we can remove $OD_2(m)$ over-estimated execution demand from $dbf_{SM}(\tau_i,\mathit{e},m)$.

% Suppose a subset of tasks  $\tau^*=\{\tau_i|d(J_i^*,m-1)\geq 0\wedge L_i\geq m \}$ is sorted by $d(J_i^*,m-1)$ (i.e, $\forall i:~d(J_i^*,m-1)\leq d(J_{i+1},m-1)$). 

Thus the available time slots $AS_i^m$ for $\tau_i$'s carry-over job $J_i^m$ can be calculated using  Equation~\ref{eqn:asm} given below. The general idea is that if $AS_i^m$ is not consumed by $J_i^m$, the remaining slots, $AS_i^m-RMD_i^m$, could be used by $J_{i+1}^m$.
\begin{equation}
\label{eqn:asm}
\begin{split}
AS_i^m=
   \begin{cases}
   d(J_i^m,m-1)&\mbox{ If } i=1\\
   d(J_i^m,m-1)-d(J_{i-1},m-1)+\max\left(0,AS_{i-1}^m-RMD_{i-1}^m\right)& \mbox{otherwise}
   \end{cases}
\end{split}
\end{equation}
\begin{equation}
\label{eqn:asm}
OD_i^m=\max\left(0,RMD_i^m-AS_i^m\right)
\end{equation}
The following lemma  then gives an upper bound of the execution demand of $\tau$ during the interval $\left[S_m,~S_m+\mathit e \right)$.
\begin{lemma}
\label{propostion:proposition1}
$dbf_{ISM}(\tau,\mathit{e},m)$ captures the maximum execution demand of task set $\tau$  in $L_m$ criticality mode for a  time interval $\left[S_m,~S_m+\mathit e\right)$, where
\begin{equation}
dbf_{ISM}(\tau,\mathit{e},m)=\sum_{L_i\geq m}dbf_{SM}(\tau_i,\mathit{e},m)-\sum\limits_{J_i^m\in J^m}\mbox{OD}_i^m
\end{equation}  
\end{lemma}
\begin{proof}
The proof for Lemma~\ref{propostion:proposition1} can be found in Section~\ref{sec:proof} in the appendix.
\end{proof}
The following theorem then follows as a straightforward extension of Theorem~\ref{theorem:theorem0}.
\begin{theorem}
\label{theorem:ISM}
A MC sporadic task system $\tau$ is schedulable by EDF on a dedicated unit speed uniprocessor platform  for all the criticality modes if the following conditions hold:
\begin{align*}
&\forall~m\in\{1,2,\ldots,M\}:~\forall \mathit{e}\in\{1,2,\ldots,\mathit e^{max}\}:~dbf_{ISM}(\tau,\mathit e,m)\leq \mathit{e}
\end{align*}
where $\mathit e^{max}$ is  pseudo-polynomial in the size of the input as given in~\cite{EkYi14}.
\end{theorem}



% The  detailed steps to calculate the overestimated demand are given in Algorithm~\ref{alg:overEst} given a task set $\tau^*$  in ascending order where $\tau^*$ is a subset of tasks with $L_i\geq m$ and  $d(J_i^*,m-1)\geq 0$.
% \begin{algorithm}[t]
% \SetCommentSty{small}
% \SetAlgoNoLine
% $\mbox{OD}^m\leftarrow 0$\tcp*[l]{\textcolor{blue}{Initially over estimated demand is equal to zero}}
% \For{$\tau_i \in \tau^*$}
% {
% 	\If{$i=1$}
% 	{
% 	$AS_1^m=d(J_1^*,m-1)$\tcp*[l]{\textcolor{blue}{For $\tau_1$, $AS_1^m=d(J_1^*,m-1)$}}
% 	}
% 	\Else
% 	{
% 	$AS_i^m=d(J_i^*,m-1)-d(J_{i-1},m-1)+AS_{i-1}^{m}$\;
% 	}
% 	\If{$AS_i^m<RMD_i^m$}
% 	{	
% 		$\mbox{OD}_{i-1}^m=RMD_i^m-AS_i^m$\;
% 		$\mbox{OD}^m=\mbox{OD}^m+\mbox{OD}_{i-1}^m$\;
% 		$AS_i^{m}=0$\;
% 	}
% 	\Else
%     {
%     	$AS_i^{m}=AS_i^m-RMD_i^m$\;
%     }
% }
% \Return $\mbox{OD}^m$\;
% \caption{Calculate overestimated execution demand: $\mbox{OD}(\tau^*, \mathit e,m)$}
% \label{alg:overEst}
% \end{algorithm}



% \begin{theorem}
% \label{theorem:theorem0}
% A MC task set $\tau$  is schedulable by EDF on a dedicated unit speed  platform for all criticality modes if the following conditions hold:
% \begin{align*}
% &\forall 1 \leq m\leq M:\mathbf{Condition~CN_m^{\mbox{\tiny{1}}}} \mathbf{ = TRUE, where }\\
% &\mathbf{Condition~CN_m^{\mbox{\tiny{1}}}}:~~\forall \mathit{e}~dbf_{ISM}(\tau_i,\mathit{e},m)(\tau,\mathit e)\leq \mathit{e}
% \end{align*}
% \end{theorem}

% \subsection{Schedulability Test}
% According to  Lemma~\ref{propostion:proposition1} Theorem~\ref{theorem:theorem0} has a natural extension:



% It is not realistic to check all the values of $\mathit e\rightarrow \infty$. Therefore here we use similar methods~\cite{BMR90} to derive the upper bound  value of  $\mathit e$ that we need to check. Let  $\mathit e_m^{max}$ denote the upper bound of $\mathit e$ in $L_m$ criticality mode.

% Assuming that we have $dbf_{ISM}(\tau_i,\mathit{e},m)(\tau, \mathit e)>\mathit e$,  $dbf^{\mbox{\tiny{GT}}}_{m}(\tau, \mathit e)\geq dbf_{m}^{\mbox{\tiny{1}}}(\tau, \mathit e)
% \Rightarrow dbf_{m}^{\mbox{\tiny{GT}}}(\tau, \mathit e)  >\mathit e$.
% Therefore we have
% \[\sum_{L_i\geq m} C_i^m \times \frac{\mathit e+T_i}{T_i}\geq dbf_{m}^{\mbox{\tiny{GT}}}(\tau, \mathit e)\geq \mathit e \]
% \[\Rightarrow \sum_{L_i\geq m} C_i^m >\mathit e- \sum_{L_i\geq m} \frac{C_i^m}{T_i} \times \mathit e\\
% \Rightarrow \mathit e <\frac{\sum_{L_i\geq m} C_i^m }{1-\sum_{L_i\geq m} \frac{C_i^m}{T_i}}\]

% Therefore the upper bound of $\mathit e$  for $dbf_{ISM}(\tau_i,\mathit{e},m)(\tau, \mathit e)$ denoted as $\mathit e^{max}_m$ is bounded by 
% \[
% \frac{\sum_{L_i\geq m} C_i^m }{1-\sum_{L_i\geq m} \frac{C_i^m}{T_i}}.
% \]

% \subsection{Introduce the  deadline  tuning algorithm}
% From the previous sections we know virtual deadlines for each criticality mode plays a key role in shaping the demand of carry-over jobs.  The choice of virtual deadline for each task has a great effect on the performance of proposed demand bound function schedulability test for MC workloads in Theorem~\ref{theorem:theorem1}. We can lessen $\tau_i$'s demand in $L_{m|m>1}$ criticality mode at the cost of increasing the demand in previous modes. By choosing suitable values for $d(J_i^*,m-1)| 2\leq m <L_i$ for all tasks $\tau_i$, we are increasing our chances to satisfy all the conditions $CN_m^1|m\in \mathcal Z^+\&  m\leq \mathcal M $ given in Theorem~\ref{theorem:theorem0}. 

% % The process of finding suitable values for the relative deadlines is very challenging because for each task $\tau_i$, the value of virtual deadline $d(J_i^*,m-1)$ is constrained to $C_i^{m-1}\leq D_i{m-1} \leq D_i^{m}\ldots\leq D_i^{L_i}$. Thus,  there will be 
% % \begin{align*}
% % \prod_{\tau_i\in \tau \& L_i\geq m}(D_i^m-C_i^{m-1}+1) 	
% % \end{align*} 
% % possible combinations, and hence it is infeasible to simply try all combinations.

% % In this section, we introduce a heuristic virtual deadline tuning algorithm to improve the performance of the demand bound function based schedulability test.

% % , and this algorithm is of pseudo-polynomial time complexity. Below we first illustrate the general ideal of this heuristic algorithm intuitively, and then present the detailed algorithm. 

% We will use Algorithm~\ref{alg:tunemode} ($TuneMode(m)^1$)  to increase the chances to satisfy condition $ \mathbf{Condition~CN_m^1}:\forall \mathit{e}:~dbf_{m}(\tau, \mathit e) \leq \mathit e $ by tuning virtual deadlines. The general idea is to check condition $\mathbf{Condition~CN_m^1}$ line~\ref{line:2} in Algorithm~\ref{alg:tunemode} for increasing time interval lengths $\mathit e$ from $0$ up to $\mathit e_{max}^m $. As soon as it finds a instance where $dbf_{m}(\tau, \mathit e) \leq \mathit e$  fails,  it chooses a candidate task with Algorithm~\ref{alg:findcandidate1} (find\_candidate\_m($\Psi$, $\mathit e$)) and reduce a candidate task's relative deadline $d(J_i^*,m-1)$ by one unit (as shown in line~\ref{line:1}) and goes back to $\mathit e=0$.

% Suppose that $dbf^1_{m}(\tau, \mathit e)>\mathit e$,  a suitable candidate task $\tau_i$  should reduce maximum demand in $L_m$ criticality mode but has the minimal impact on the schedulability in $L_{m-1}$ criticality mode. Let $\Delta_i=dbf_{m}(\tau_j,\mathit e)- dbf_{m}(\tau_j,\mathit e)|_{d(J_i^*,m-1)\leftarrow d(J_i^*,m-1)-1}$, then a task $\tau_i$ which has the maximum $\Delta_i|_{\Delta_i>0}$ is preferred. However in case there is no such task with $\Delta_i>0$, then a task with minimal $len_i\leftarrow mod(\mathit e,T_i)-(D_i^{m}-d(J_i^*,m-1))-C_i^{m-1}$ is preferred.  Here $len_i$ denotes the minimal amount that $d(J_i^*,m-1)$ need to decrease so that   $dbf_{m}(\tau_j,\mathit e)$  can be tuned.

% \begin{algorithm}[t]
% \SetCommentSty{small}
% \SetAlgoNoLine
% \KwIn{Candidate task set $\Psi$}
% \KwOut{Candidate task index}
% \CommentSty{\color{blue}}
% $Q\leftarrow \mbox{empty queue}$\;
% \For{$\tau_i  \in \Psi$}
% {
% 	$len_i\leftarrow mod(\mathit e,T_i)-(D_i^{m}-d(J_i^*,m-1))-C_i^{m-1}-1$
% 	$\Delta_i\leftarrow dbf_{m}(\tau_i,\mathit e)-dbf_{m}(\tau_j,\mathit e)|_{d(J_i^*,m-1)\leftarrow d(J_i^*,m-1)-1}$\;
% 	$Q.insert((\Delta_i,len_i,A))$\;


% }
% $Q.sort(\{\Delta_i\mbox{:ascending}\},\{l_i^{m-1}\mbox{:descending}\})$ \tcp*[l]{\textcolor{blue}{sort tasks in $\Psi$ with first key $\Delta_i$ in ascending order and then with second key $l_i^{m-1}$ in descending order}}
% index $\leftarrow Q.\mbox{pop()}$\;
% \Return index
% \caption{find\_candidate\_m($\Psi$, $\mathit e$)}
% \label{alg:findcandidate1}
% \end{algorithm}






% Algorithm~\ref{alg:tunemode} ($TuneMode(m)^1)$ decreases the relative deadlines of tasks i.e., $d(J_i^*,m-1)$, to reduce the demand of those tasks in the successor mode i.e., $L_{m}$ criticality mode. It does this without considering of the schedulability in $L_{m-1}$ criticality mode itself, hoping that $\tau$ in  $L_{m-1}$  criticality mode can later be made schedulable by decreasing deadlines for $L_{m-2}$ criticality mode i.e., $D_i^{m-2}$. Once $d(J_i^*,m-1)$ decreases to $C_i^{m-1}$ but  $dbf^1_{m}(\tau, \mathit e)>\mathit e$ still holds, then $\tau_i$ is eliminated from the candidate sets $\Psi_m$ in line~\ref{line:3}, and then we need to find another candidate task. We can repeat the above steps  until  $dbf^1_{m}(\tau, \mathit e)\leq \mathit e$ becomes true or the candidate task set $\Psi_m$ becomes empty. 

% A exceptional case is that: if we reduce $D_i^1$ to lessen the demand in $L_2$ criticality mode, $\tau$ may become unschedulable in $L_1$ criticality mode. However there does not exist $D_i^0$, and we cannot tune $D_i^0$ to lessen the demand in  $L_1$ criticality mode. Therefore in this case, $TuneMode(m)^1$ will undo changes to deadlines that would make $\tau$ unschedulable in $L_1$ criticality mode. 



% \begin{algorithm}[t]
% \SetAlgoNoLine
% \SetCommentSty{small}
% \caption{$TuneMode(m)^1$}
% $mods\leftarrow \mbox{empty stack}$\;
% $\Psi_m\leftarrow \{i|L_i\geq m\}$\;
% \For{$\tau_i \in \Psi_m$}
% {
% 	$d(J_i^*,m-1)\leftarrow D_i^{m}$\;
% 	\If{$d(J_i^*,m-1)=C_i^{m-1}$}{$\Psi_m=\Psi_m.remove(\tau_i)$\;}
% 	\If{$d(J_i^*,m-1)<C_i^{m-1}$}{\Return $\mathbf{False}$\;}
% }
% $changed\leftarrow\mathbf{False}$\;
% \While{$changed=\mathbf{True}$}
% {
% 	$changed\leftarrow \mathbf{False}$\;
% 	\For{$\mathit e= 1,2,\ldots,\mathit e_{max}^m$}
% 	{	
% 		\If{$m=2$ and $dbf^1_{m-2,m-1}(\tau, \mathit e)>\mathit e$}
% 		{
% 			undo the deadline change and remove the candidate task from $\Psi_m$ by calling function undo()\;
% 			% \If{$mods$ is empty}{\Return $\mathbf{False}$\;}
% 			% $i\leftarrow mods.pop()$\;
% 			% $d(J_i^*,m-1)\leftarrow d(J_i^*,m-1)+d(J_i^*,m-1)+1$\tcp*[l]{\textcolor{blue}{undo the changes to the deadlines}}
% 			% $\Psi_m.remove(i)$\;
% 			% $changed\leftarrow \mathbf{True}$\;
% 			% \textbf{break}\;
% 		}
% 		\If{$dbf^1_{m}(\tau, \mathit e)>\mathit e$\label{line:2}}
% 		{
% 		\If{$\Psi_m=\emptyset$}{\Return $\mathbf{False}$\;}
% 		$i\leftarrow find\_candidate^2(\Psi_m, \mathit e, m)$\;
% 		$d(J_i^*,m-1)=d(J_i^*,m-1)-1$\;\label{line:1}
% 		$mods.push(i)$\;
% 		\If{$d(J_i^*,m-1)\leq C_i^{m-1}$}
% 		{
% 		$\Psi_m.remove(i)$\label{line:3}\tcp*[l]{\textcolor{blue}{If $d(J_i^*,m-1)\leq C_i^{m-1}$, $i$ is removed from $\Psi_m$}}

% 		}
% 		$changed\leftarrow \mathbf{True}$\;
% 		\textbf{break}\;
% 		}

% 	}
	
% }
% \Return $\mathbf{True}$
% \label{alg:tunemode}
% \end{algorithm}




% Algorithm~\ref{alg:tunesystem} ($TuneSystem(\tau)$)   apply   Algorithm~\ref{alg:tunemode}  ($TuneMode(m)^1$) on all the criticality modes starting from $L_{\mathcal M}$ criticality mode and proceeding in a reverse order until it has successfully tuned all criticality modes or failed in tuning some criticality mode. 
% \begin{algorithm}[t]
% \SetCommentSty{small}
% \SetAlgoNoLine
% \KwIn{Taskset $\tau$}
% \KwOut{$\mathbf{True}$ or $\mathbf{False}$}
% $\mathcal M\leftarrow\max_{\tau_i\in \tau}\{L_i\}$\tcp*[l]{\textcolor{blue}{$TuneMode(m)^1|m>2$ will check the schedulability for $L_m$ criticality mode, $TuneMode(1)$ will check the schedulability for both $L_2$ and $L_1$ criticality mode.}}
% \For {$m\in \{\mathcal M~\mbox{to}~1\}$} 
% {
% 	\If {$TuneMode(m)=\mathbf{false}$}
% 	{
% 		\Return $\mathbf{false}$
% 	}
% }
% \Return $\mathbf{True}$
% \caption{TuneSystem($\mathcal{T}$)}
% \label{alg:tunesystem}
% \end{algorithm}





















==> response.tex <==

% \section{Response To Comments}

\noindent Dear Editor/Reviewers,\\\\

\noindent Please find the attached revision of our paper, titled ``Efficient Schedulability Test for Dynamic-Priority Scheduling of MC Real-Time Systems".\\


\noindent We thank the reviewers for their time and the valuable comments, which greatly help improve the quality of the paper.  We have tried to address all their concerns, and  hope that our responses could address their concerns in a satisfactory way.\\


\noindent Thank you for your consideration,\\

\noindent Xiaozhe Gu and Arvind Easwaran

\subsection{Major Changes}
Before we provide specific responses to the reviewers, here we first list all the major changes done to the draft.\\

\begin{itemize}
  \item  From \lr{mj1s} to \lr{mj1e}, we present a  discussion  about the shortcomings of the SM dbf test~\cite{EkYi14} and the challenge in extending the initial result  in ~\cite{Eas13} to  multi-criticality systems.
  \item From \lr{mj2s} to \lr{mj2e}, we use a new example  to demonstrate the drawback of the SM dbf in \cite{EkYi14}.
  \item  From \lr{mj3}, we add a short discussion about the challenge in  extending the MM dbf test to a more generalized model.

  \item From \lr{mj4s} to \lr{mj4e}, we explain the simple metric  that \cite{EkYi14} uses for choosing candidate tasks. Then we introduce our new metric to choose candidate tasks and present the insights about why the new metric can further improve schedulability.
  \item In Section~\ref{sec:eva}, we first change the bar plots to line plots. We add the results of the SM dbf test in  \cite{EkYi14} with our new metric to choose candidate tasks in order   to demonstrate the effectiveness of the new metric. We remove the results of EDF-VD and AMC  and merge some figures to save space and focus on comparison with  \cite{EkYi14}. To better demonstrate how the acceptance ratio changes as the number of criticality levels increases, we also show the weighted acceptance ratios when the  number of criticality levels is equal to 2, 3, 4, 5.
\end{itemize}



\subsection{Referee: 1}
Major Issues.
\begin{itemize}
  \setlength\itemsep{1em}
\item It is not clear what the main technical contributions are in the new formulation of the demand bound functions. The experiments show that there are pragmatic improvements here, but please try to clarify what the main new insights of this paper are, given the previous results of ~\cite{Eas13} and~\cite{EkYi14}\\

\bg{ Response: The SM dbf in \cite{EkYi14} is presented in Section~\ref{sec:ExistDBF} which is totally different from the MM dbf  in  this paper.  When the criticality level=2, the MM dbf in this paper and ~\cite{Eas13} are the same. However, as pointed in the introduction section, there are two challenges in extending the MM dbf in \cite{Eas13} to multi-criticality systems. First, the pattern that can result in maximum demand in  \cite{Eas13}  is no longer valid in multi-criticality systems because   \cite{Eas13} only consider two levels, i.e., it only considers the case when there is  one mode-switch. As a result,  it does not need to consider the demand of jobs released before $S_{m-1}$ but have deadline after $S_{m-1}$ (i.e., $J_i^A,J_i^C$).  The MM dbfs in Section~\ref{sec:GIT} derive $dbf_{MM}(J_i^A/J_i^C,S_m,\mathit e,m)$.  Finally,  we  cannot consider the demand from the start of a busy interval as \cite{Eas13} does, because in this case,  we have to consider  all possible combinations of the values of  mode-switch instants, and the complexity of the test is exponential in the number of criticality levels. Therefore, in this paper, we consider the demand from the previous mode-switch instant $S_{m-1}$.  This paper also improves the strategy in ~\cite{EkYi14}  for choosing  candidate tasks (details are given in Section \ref{sec:T1}). Finally, we combine the SM dbf test and MM dbf test by using the MM dbf test as a complement to further reduce the computation time of the MM dbf test.}\\

\item  The tuning algorithms TuneSystem and TuneMode seem like straightforward extensions of the algorithms with the same names in \cite{EkYi14}. I would refrain from referring to them as "novel".\\

\bg{Response: Although the general objective of the tuning algorithms are similar to those presented in \cite{EkYi14}, there are several important differences. First, we have used a metric to choose a candidate task based on the maximum change in SM dbf (similar to the metric used for dual-level systems in \cite{EkYi12}). Second, we also use another metric $D_i^{m-1}$ to further differentiate between the candidate tasks. Because a larger $D_i^{m-1}$ can increase the chances that the system is schedulable in previous mode. Finally, we also consider the case when there does not exist a candidate task so that the total demand would decrease if $D_i^{m-1}\leftarrow D_i^{m-1}-1$. In this case,  we choose a task  that requires  minimal steps of tuning. These aspects of the tuning algorithms are discussed in detail in Section ~\ref{sec:T1}.   Besides, unlike the tuning algorithm in \cite{Eas13,EkYi12} where either SM or MM dbf test is used, we use MM dbf test as a complement for SM dbf test to reduce the computation time of the MM dbf test.  In the evaluation section, we present additional results that clearly show the benefits of the tuning algorithms over existing ones.   }\\

\item As the express purpose of this paper is to improve upon the results of \cite{EkYi14}, you should also mention that those previous results address a much more expressive task model than this paper. Please also add a discussion about whether your approach would also work for the more general
model.\\

\bg{Response: a short discussion is added at the end of Section~\ref{sec:GIT}. The MM dbf derived in this section cannot directly be applied to  a more generalized MC model where each task has different periods in different criticality modes. The challenge in this extension is that we need to consider more cases and derive the new release pattern, i.e., the release time of $J_i^A$ and $J_i^C$,  that  can result in the maximum demand. Of course, we can still compute the demand for all possible release patterns and choose the maximum one, but it can be very computational expensive. For space reason, we would leave this as our future work.
}\\

\item To make a stronger point about this approach being scalable, I recommend adding some plot for comparing the running times of the considered schedulability tests.\\

\bg{Response:  The complexity of Algorithm~\ref{alg:tunemode} is independent of the criticality levels (i.e., the value of m). Therefore, we can find the complexity of Algorithm~\ref{alg:tunesystem} increases linearly as the number of criticality level (i.e., the value of $M\leftarrow\max_{\tau_i\in \tau}\{L_i\}$) increases. Compared to \cite{EkYi14}, there is a  there is a quadratic increase in complexity.}\\

\end{itemize}


Minor Issues.

\begin{itemize}
  \setlength\itemsep{1em}
  \item  I would not refer to running schedulability tests on random task sets as "simulation".\\

  \bg{Response: we use ``experiment" to replace it.}
  \item Page 3, line 5: "GreedTuning" to "GreedyTuning" . \\ \bg{Response:~We have changed it as you suggested.}
  \item Page 3, line 48: "e.e." to "e.g." \\ \bg{Response:~We have changed it as you suggested.}
  \item  Page 4, line 40:  releases an infinite sequence to releases a potentially  infinite sequence (or perhaps unbounded). \\  \bg{Response:~We have changed it as you suggested.}
  \item  Page 4, line 50: $>=$ to    $\geq$.\\ \bg{Response:~We have changed it as you suggested.}

  \item  The notation with a vertical bar $|$ to mean "such that" that is used throughout the paper is non-standard outside of set-builder notation. I recommend you write out "such that" instead.\\ \bg{Response: We avoid using $|$  now}.

  \item  What is motivation for using "e" to denote interval lengths, as opposed to more established notation? \\ \bg{Response: We use $\mathit e$ in order to be consistent with the previous work \cite{EkYi14} where $\mathit e$ is used to denote the time interval length.}
  \item  Definition 2.2 is a non-definition. It defines a concept in terms of other
  non-defined concepts.
  
  \bg{Response: we have given a more detailed definition about dbf: A demand bound function $dbf(\tau_i,\mathit e)$ gives an upper bound on the maximum possible execution demand of task $\tau_i$ in any time interval of length $\mathit e$, where demand is calculated as the total amount of required execution time of jobs with their whole scheduling windows within the time interval.}\\

  \item You should mention that Eq. (1) as stated is only for constrained deadlines.\\ \bg{Response:We add it is ``for non-MC constrained deadline task model" before Eq. (1).}

  \item  About the notation on line 31, page 4: First, ${C_i^1, ..., C_i^{L_i}}$ is not
  an element of $N^{+}$. Second, you probably want $C_i$ to be a tuple, not a set 
  (it is then an element of $(N^{L_i})$.\\ \bg{Response: we change it to `` $C_i=(C_i^1,~C_i^2,\ldots,C_i^{L_i})$ is a $L_i$-tuple of estimated execution time budgets respectively for each criticality level''}


  \item In many places (e.g., Theorem 3.1, Theorem 4.1 and Section 5) you state that
  $e_{max}$ is a pseudo-polynomial in the size of the input. This is *only* known
  to be true if the utilization is bounded by some constant smaller than 1.\\
  \bg{Response: we have added the condition ``if the system utilization of each criticality mode is  bounded by some constant smaller than 1" before the  statement.}\\



  \item  Please be clearer in that all of Section 3 is summarizing a previous paper.\\ \bg{Response: We mention that the SM dbf is from an existing work~\cite{EkYi12} at the beginning of Section 3.}

  \item  Page 7, line 27: "should happen" to "could happen". \\\bg{Response: We have changed it as you suggested.}

  \item  The issues you detail about the SM dbf test on the top of page 9 are mostly
  occurring because you assume there that no deadline tuning has taken place.
  Perhaps another example would better demonstrate the actual benefits of the
  MM dbfs

  \bg{Response: we have presented another example.}

  \item  First paragraph of page 19: Here it sounds as if you can easily compute the  demand of carry-over jobs, instead of an easily-computed over-approximation  of that demand. Those are very different things.\\
  \bg{Response: Is the page number wrong? We do not talk about dbf for carry-over job there. The  dbf of carry-over jobs upper bound the demand of these jobs and it is an over-approximation. We use ``a bound of the demand of  carry-over  jobs" to replace  the  ``demand of carry-over jobs".}

  \item  Fig. 5: $L_i = m$ should be $L_i \geq m$? \bg{Response: We have changed it.}

  \item Page 10, line 43 and page 11, line 48: $\{0, 1, 2, ..., T_i\}$ should be  $\{0, -1, -2, ..., -T_i\}$? \bg{Response: it should be $\{0, -1, -2, ..., -T_i\}$, we have changed them now.}

  \item  Algorithm 1 can be better expressed. How do you "undo" the changes at line 9?  What is the use of the stack "mods"?\\
  \bg{Response: we have removed mods now. The undo means: $D_i^{1}\leftarrow D_i^{1}+1$ and
      $\Psi_m$.remove($\tau_i$).  We have modified this part in Algorithm 1 now.  }

  \item  This is a matter of taste, but I think line plots would be much easier to read than histograms for your experiments.\\ \bg{Response:~We have used line plots now.}

  \item  Appendix: Why do section numbers start with a dot?\\ \bg{Response:~We have changed it as you suggested.}

  \item Page 19, line 44: Sectio to Section.\\ \bg{Response:~We have changed it as you suggested.}

  \item  Page 20, line 29: $C_i^{m-1}$ should be $C_i^{m-2}$?\\ \bg{Response: It should be  $C_i^{m-2}$.}


\end{itemize}





\subsection{Referee: 2}


\begin{itemize}
  \setlength\itemsep{1em}
\item  For the paragraph above Theorem 4: the reviewer did not follow why dbf is independent of $S_{m-1}?$ Can you provide more explanations?! \\ \bg{Response: We  are interested in the demand of $\tau_i$ during $[S_{m-1}, \mathit {e}]$. As introduced in Section~\ref{sec:GIT}~\lr{Ind},  the time interval length  $\mathit e$ and $S_m-S_{m-1}$  determine the total the demand, and hence   exact value of $S_{m-1}$ does not influence the total demand.}

\item page 13, 2nd paragraph: what is “one unit”? How is the complexity of the algorithm related to the unit?\\ \bg{Response: In the footnote of ~\lr{integer}, we point out  that we focus on integer release model, i.e.,  $T_i,~D_i \in \mathbb Z^+$, and hence $D_i^m$ is also assumed to be integer value.}
\item section 6.1: what is RD for?! \\ \bg{Response: RD is a parameter used to set the deadline of tasks, i.e., the deadline $D_i\in \left[\lfloor C_i^{Li}+RD\times(T_i-C_i^{L_i}) \rfloor,T_i\right]$}

\item    .. redundant phrase in the two lines below Algorithm 3; \\ \bg{Response: We removed the redundant part.}
\item    .. page 9, 3rd para, line 2: the *n* demand?! \\ \bg{Response: We removed  "n"}

\item    .. page 5, Definition 2.1: “… while the system stays in $L_m$ criticality mode”.           note that, some of the execution of $C_i^m$ may run at a lower criticality levels?!        This part needs rephrase to reflect such facts. \\ \bg{Response:  Yes, some execution of $C_i^m$ may run at lower criticality levels. Suppose the system switches to $L_m$ mode at $t^*$, by $t^*$,  a job may already have executed for some time but this execution cannot exceed $C_i^{m-1}$ because otherwise the system would already switch to $L_m$  criticality mode before $t^*$ (see \lr{m1}).   


 }

\end{itemize}



\subsection{Referee: 3}

\begin{itemize}
  \setlength\itemsep{1em}
  \item For the improved test, it is actually not clear what exactly are the new contributions as compared to the authors' own previous work and those work from the others. It seems that they straightforwardly applied their dual-mode analysis to multi-mode, since any mode transition is equivalent to a dual-mode transition.\\ 
  \bg{Response: 
The SM dbf in \cite{EkYi14} is presented in Section~\ref{sec:ExistDBF} which is totally different from the MM dbf  in  this paper.  When the criticality level=2, the MM dbf in this paper and ~\cite{Eas13} are the same. However, as pointed in the introduction section, there are two challenges in extending the MM dbf in \cite{Eas13} to multi-criticality systems. First, the pattern that can result in maximum demand in  \cite{Eas13}  is no longer valid in multi-criticality systems because   \cite{Eas13} only consider two levels, i.e., it only considers the case when there is  one mode-switch. As a result,  it does not need to consider the demand of jobs released before $S_{m-1}$ but have deadline after $S_{m-1}$ (i.e., $J_i^A,J_i^C$).  The MM dbfs in Section~\ref{sec:GIT} derive $dbf_{MM}(J_i^A/J_i^C,S_m,\mathit e,m)$.  Finally,  we  cannot consider the demand from the start of a busy interval as \cite{Eas13} does, because in this case,  we have to consider  all possible combinations of the values of  mode-switch instants, and the complexity of the test is exponential in the number of criticality levels. Therefore, in this paper, we consider the demand from the previous mode-switch instant $S_{m-1}$.  This paper also improves the strategy in ~\cite{EkYi14}  for choosing  candidate tasks (details are given in Section \ref{sec:T1}). Finally, we combine the SM dbf test and MM dbf test by using the MM dbf test as a complement to further reduce the computation time of the MM dbf test.}\\



  \item The authors mentioned some complexity problems with their own old test, however the improvements are not very clearly elaborated and lost in all the formal equations. More explanations and possible re-organizations are needed to show the complexity reductions.  \\
  \bg{Response: we add a discussion  in introduction:  we  cannot consider the demand from the start of a busy interval as \cite{Eas13} does, because there would be  multiple mode-switches, e.g., $S_1,~S_2,\ldots,S_m$  in the time interval. In this case, we have to consider  all possible combinations of the values of $S_1,~S_2,\ldots,S_m$, and as a result,  the complexity of the test is exponential in the number of criticality levels. To reduce complexity, in this paper, we consider the demand from the previous mode-switch instant $S_{m-1}$. As a result, we only need to consider the demand when  $S_m$  have different values. }

  \item   The authors motivated the new test from a complexity point of view (exponential in the number of criticality levels). However, realistic systems only have less than 5 criticality levels. Would this be really an issue? By reducing the complexity, how much pessimism do you introduce into the new test? \\ \bg{Response: As pointed in the introduction, reducing the complexity is just one challenge if we directly use the insights of  \cite{Eas13} for multi-criticality systems ,i.e., analyze the system from the start of a busy interval rather than from  a mode-switch instant.   However, as discussed in the earlier response related to “new contributions”, the insights of \cite{Eas13} cannot be directly extended to multi-level systems. We still need to determine the pattern across multiple mode-switch instants that would maximize demand in the interval of interest. How to determine this pattern without introducing significant pessimism across each mode-switch is not known. So, it is not clear that the additional complexity (exponential in the number of criticality levels) would always result in reduced pessimism.  

 }

  \item The explanation of the deadline tuning algorithm needs to be extended and to be more clear. Currently, it is very short and hard to follow what are the new ideas in the optimization compared to old ones.   Also, you should try to minimize formal equations in your explanation and use plain language instead. You can start with a general intuitive explanation about the shortcomings of existing optimizations, your main idea to develop a new one, and the major steps of your algorithm. Then you could go to the details. \\
  \bg{Response:  First, we introduce that, unlike the tuning algorithm in \cite{Eas13,EkYi12} where either SM or MM dbf test is used, we use MM dbf test as a complement for SM dbf test (as shown in line 18-27 in Algorithm~\ref{alg:tunemode}) to further reduce the computation time of MM dbf test.

  Besides, we have introduced the only metric that ~\cite{EkYi12} uses to choose a candidate task, i.e.,  task $\tau_i$ with $\Delta_i=\max\{dbf_{SM}(\tau_i,\mathit e,m)-dbf_{SM}(\tau_i,\mathit e-1,m)\}$ is always chosen as a candidate task in \lr{Tune1}.  However, the value of  $D_i^{m-1}$  is  also important metric, and we use a simple example motivate  that a candidate task with larger  $D_i^{m-1}$ can increase the chances that the system is schedulable in previous mode  (from \lr{tune2}). From \lr{tune3}, we also mentioned that the new candidate task choosing algorithm also considers how to choose a candidate task  when there does not exist a task so that the total demand would decrease if $D_i^{m-1}\leftarrow D_i^{m-1}-1$. In this case, it will choose a task  that requires  minimal steps of tuning before the total demand would decrease. }

  \item The figures in the experiments are difficult to digest due to the use of bar-plot - it is not easy to compare the trends of different approaches. Why don't you use line-plot instead? Is there any reason that instead bar-plot is chosen?\\ \bg{Response: We use line-plot now.}

  \item You should explicitly say that less critical tasks are dropped in hi mode (at least do not interfere with hi task executions, and use similar extensions with multi-mode). Otherwise, the analysis would be wrong.  \\  \bg{Response: we add  "After this mode switch at $S_m$, jobs with criticality level $L_i<m$, including those that were released before $S_m$ but did not complete until $S_m$,  are no longer required to meet deadlines. For simplicity of analysis, these jobs are assumed to be dropped thereafter" in Section~\ref{sec:model}}


\item  Page 1. It is not clear the relationship between open systems and mixed-criticality systems. Many mixed-criticality system are indeed not open and do not need to be. They are different concepts that possibly overlap. Please reformulate to make your statement more accurate. \\ \bg{Response: We  avoid using the concept ``open systems" now.}

  \item Page 2. The interpretation of criticality in the research community is controversial. It is not necessary that a high critical one fails with a more severe consequence as the industry takes many other factors into account when define criticality.\\  \bg{Response: That's true, and here  we add  "typically" before the statement.}

  \item Page 3. unclear statements: "use very conservative assumptions", "the system in each criticality", "the complexity is exponential"... Can you please be more precise?\\ 
      
               \begin{enumerate}
                 \setlength\itemsep{1em}
                \item ``use conservative assumptions":  \bg{As we pointed in  Section~\ref{sec:intro} and \lr{pess1}, the SM dbf conservatively assuming maximum carry-over demand when the system behavior switches from a lower criticality level to the one being analyzed. However, the actual carry-over demand could be much lower.}

                \item ``They separately analyze the system in each criticality level": \bg{ The details of  SM dbf is introduced in Section~\ref{sec:ExistDBF}.  In  \lr{spe} we pointed out that, SM dbf bound the demand during  $[S_m,S_m+\mathit e)$, and only consider the time interval after a mode-switch $S_m$, but what happened before $S_m$ is totally ignored.}
                
                \item "the complexity is exponential":  \bg{We pointed out in Section~\ref{sec:intro} \lr{intro1} that,  if we directly use the insights of the work \cite{Eas13}, i.e.,  consider the demand from the start of a busy interval. Then there would be  multiple mode-switches, e.g., $S_1,~S_2,\ldots,S_m$  during the time interval. In this case, we have to consider  all possible combinations of the values of  $S_1,~S_2,\ldots,S_m$   and as a result,  the complexity of the test is exponential in the number of criticality levels.}
                \end{enumerate}
  

  \item Page 4. Similar to Page 3: "there is a significant gap", good, bad? \\ \bg{Response: we use "outperforms other techniques " instead.}

  \item Section  in Appendix to Appendix  \\ \bg{Response:  We have changed it as you suggested.}

 
\end{itemize}
















==> test.tex <==
\appendix
\section{Proofs}
\label{sec:proof}
$dbf^{\mbox{\tiny{1}}}_{m}(\tau, \mathit e)$ captures the maximum execution demand of task set $\tau$  in $L_m$ criticality mode for a  time interval length equal to $\mathit e$ where,
\begin{equation}
dbf^{\mbox{\tiny{1}}}_{m}(\tau, \mathit e)=\sum_{\tau_i\in \tau\wedge L_i\geq m}dbf^{\mbox{\tiny{GT}}}_{m}(\tau_i,\mathit{e})-\mbox{OD}(\tau, \mathit e,m)
\end{equation}  
\begin{proof}
Suppose $dbf^{\mbox{\tiny{1}}}_{m}(\tau, \mathit e)$ is not an upper bound of the execution demand of task set $\tau$ for a time interval length $\mathit e$ in $L_m$ criticality mode, then there must exist other job release pattern which implies a higher bound of the total execution demand. Such a job release pattern implies that there exist at least one task $\tau_i$ whose last job $J_i^L$ released in the time interval $[0,\mathit e)$ has $d(J_i^L,m)=r(J_i^L)+D_i^m-\mathit e=x\neq0$.



% Suppose  $RMD_i^m\leftarrow RMD_i^m+\Delta RMD_i^m$, then $\Delta RMD_i^m=\Delta OD_i^m+
% |\Delta AS_{i+1}^m|\geq \Delta OD^m$.  Suppose $d(J_i^*,m-1)\leftarrow d(J_i^*,m-1)+|x_1|$ so that $ d(J_{j-1}^*,m-1)\leq d(J_i^*,m-1)\leq  d(J_j^*,m-1)$. Then 


\begin{figure}[th]
\centering 
  \includegraphics[scale=0.7]{fig3/p1}
\caption{Job release pattern ($d(J_i^L,m)\neq \mathit e$)}
\label{fig:p1}
\end{figure}
As shown in Figure~\ref{fig:p1}, we categorize the such patterns into two cases: (\textbf{P1}) $d(J_i^L,m)-\mathit e_1=x_1<0$ and (\textbf{P2}) $d(J_i^L,m)-\mathit e_2=x_2>0$. Note that the original pattern in this Lemma is $d(J_i^L,m)=\mathit e_0$ and is denoted as  \textbf{P0}. 





\textbf{P1}: As we shift the original job release pattern (\textbf{P0}) right with $|x_1|$ (i.e., the release time of all jobs increases by $|x_1|$)  so that $d(J_i^L,m)<  \mathit e_1\rightarrow d(J_i^L,m)=\mathit e_1$, then $\Delta dbf^{\mbox{\tiny{GT}}}_{m}(\tau_i, \mathit e)=IN_i\geq \Delta RMD_i^m \geq 0$, because as $r(J_i^*)$ increases,  its execution demand would only increase or stay the same. First if $RMD_i^m$ increase by  $\Delta RMD_i^m$, then $\Delta \mbox{OD}^m\leq \Delta RMD_i^m$. Second if $d(J_i^*,m-1)$ increase by  $|x_1|$, $\Delta \mbox{OD}^m\leq 0$.  Therefore by shifting  original job release pattern (\textbf{P0}) right with $|x_1|$, $\Delta \mbox{OD}_m\leq IN_i$. As we shift to $\tau_i$'s release pattern (\textbf{P1}) to  \textbf{P0}, $\Delta \mbox{OD}_m+IN_i\geq 0$ and the total demand increases or stay the same. By repeating such steps,  the total demand would increase or stay the same.





% Two steps: 1 if RMD_i increase by $IN_i$ but d_i^m does not change, OD would increase by at most IN_i 
%2. if RMD_i not change and  shift d_i^m right, the OD would only decrease or stay the same 
% As $d(J_i^*,m-1)$ does not increase but $RMD_i^m$ increase by  $\Delta RMD_i^m$ then $\Delta \mbox{OD}_m\leq \Delta RMD_i^m$. Besides if $RMD_i^m$ stays the same but $d(J_i^*,m-1)$ increases, $ \mbox{OD}_m$ would decreases or stay the same.



\textbf{P2}: As we shift the original job release pattern left with $x_2$ so that $d(J_i^L,m)>\mathit e_2\rightarrow d(J_i^L,m)=\mathit e_2 $ (i.e., release time of all jobs decreases by $x_2$). 
If  \textbf{P2.1} $\mathit e \geq D_i^m$  the demand of the last job will increase with $C_i^m$ while the demand of the carry-over job $J_i^*$ could decrease with $DE_i|\in [0,C_i^m]$. Meanwhile the overestimated demand would increases by at most $C_i^m-DE_i$ due to $d(J_i^*,m-1)$ decreases by $x_2$.  Thus by repeating shift release pattern of such tasks, the total demand would only increase or stay the same. 
\begin{figure}[h]
\centering 
\includegraphics[scale=0.7]{fig3/p2.pdf} 
\caption{Pattern 2.2}
\label{fig:p2}
\end{figure}

On the other hand if \textbf{P2.2} ($D_i^m-D_i^{m-1} \leq \mathit e \leq D_i^m$) as shown in Figure~\ref{fig:p2}, $\tau_i$ generates $0$ demand. Thus as we shift the release pattern left by $x_2$, the total demand would increase or stay the same.

 % then as we shift  $r(J_i^*)$ left by $x_2$, thus the demand of $J_i^*$ may stay the same (if $r(J_i^*)-x_2+D_i^{m-1}<S_m=0$) or increase by $C_i^m-C_i^{m-1}+\min\{r(J_i^*)-x_2+D_i^{m-1},C_i^{m-1}\}$.  Meanwhile the overestimated demand  $OD^m$ would also remain the same or increase by at most $\{r(J_i^*)-x_2+D_i^{m-1},C_i^{m-1}\}$. Thus by repeating such steps  to shift release pattern for all such tasks, the total demand would remain the same or increase.  

Finally we do not to consider the case \textbf{P2.3} ($\mathit e <D_i^m-D_i^{m-1}$) because in this case $\tau_i$ would not generate any demand in the time interval anyhow.
Therefore in sum  we can claim that the assumption is invalid, and Lemma~\ref{propostion:proposition1} is true.
\end{proof}






Task $\tau_i|_{L_i=m-1}$ generates maximum demand during $[S_{m-1},S_m)$ if  $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}$  or $r(J_i^{*_A})=mod(\mathit e- D_i^{m-1},T_i)-T_i$ (i.e.,  the deadline of job $d(J_i^{*_{A}},m-1)/d(J_i^{*_{B}},m-1)=\mathit e$), and all the jobs are released as soon as possible with period $T_i$. 
\begin{proof}
% From Lemma~\ref{lem:pat1} we know that $\tau_i$ generates maximum demand if all the jobs are released with period $T_i$ for a fixed $r(J_i^A)$, and hence we need the find the $r(J_i^A)$ so that $\tau_i$ can generate maximum possible demand. while

We know $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)|L_i=m-1$ is equal to $dbf(J_i^{*_A},S_m,\mathit e)+C_i^{m-1}\times n_{m-1}+dbf(J_i^{*_B},S_m,\mathit e)$ if $r(J_i^{*_{A+1}})< S_m$ or $dbf(J_i^{*_A},S_m,\mathit e)$ otherwise.  

First if $(\mathit e\leq D_i^{m-1})$, obviously $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)$ maximizes when  $r(J_i^{*_A})=mod(\mathit e- D_i^{m-1},T_i)-T_i$, i.e., $d(J_i^{*_A},m-1)=\mathit e$.

Second if $(S_m\leq C_i^{m-1}\wedge \mathit e> D_i^{m-1})$, we can find $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)$ maximizes when $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}$, and $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)=S_m$. Therefore we can exclude the above two simple cases now, and in the following part we only need to consider case when $\mathit e> D_i^{m-1} \wedge S_m> C_i^{m-1}$. 


% Assuming initially $r(J_i^{*_A})=-T_i$, and we shift the  job release pattern of $\tau_i$ so that $r(J_i^{*_A+1})\in(-T_i,0)$. 

% As $r(J_i^{*_A})$ increases, $dbf(J_i^{*_A},S_m,\mathit e)$ would increase from $0$ to $C_i^{m-1}-C_i^{m-2}$   (if $r(J_i^{*_A})=-D_i^{m-2}$), and then increase linearly from $C_i^{m-2}$ to $C_i^{m-1}$ when  $r(J_i^{*_A})\in [-D_i^{m-2},-D_i^{m-2}+C_i^{m-2}]$. Meanwhile $dbf(J_i^{*_B},S_m,\mathit e))$ may stay the same (if $r(J_i^{*_B})+C_i^{m-1}<S_m$ or decrease linearly ($r(J_i^{*_B})+C_i^{m-1}>S_m$) or decrease to zero (if $r(J_i^{*_B})+C_i^{m-1}>\mathit e$).  

Suppose initially $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}$, and  $r(J_i^{*_B})+D_i^{m-1} \leq \mathit e$. As we shift the release pattern left, i.e., $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}+x|x<0$, we can find that the decrease in $dbf(J_i^{*_A},S_m,\mathit e)$  ($|\Delta_1(x)|$) is  would be always  greater than the increase in $dbf(J_i^{*_B},S_m,\mathit e)+C_i^{m-1}\times n_{m-1}$ ($\Delta_2(x)$), i.e., 
\[
 \Delta_1(x)+ \Delta_2(x)\leq 0 
\]
As we shift the release pattern right, i.e., $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}+x|x\geq 0$,  $\Delta_1(x)=0$ and $\Delta_2(x)\leq 0$.  Therefore if $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}$, and  $r(J_i^{*_B})+D_i^{m-1} \leq \mathit e$,  $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)|L_i=m-1$ maximizes when $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}$. 

However if initially $r(J_i^{*A})= -D_i^{m-2}+C_i^{m-2} $ but $r(J_i^{*_B})+D_i^{m-1} > \mathit e$. As we shift the release pattern right, i.e., $r(J_i^{*A})= -D_i^{m-2}+C_i^{m-2}+x|x\geq 0$, then again $\Delta_1(x)=0$ and $\Delta_2(x)\leq 0$.

On the other hand As we shift the release pattern left, i.e., $r(J_i^{*A})= -D_i^{m-2}+C_i^{m-2}+x|x<0$,  $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)$ will first decrease linearly and then decrease to zero immediately, i.e., 
\[
\begin{split}
	\Delta_1(x)
   \begin{cases}
	x &\mbox{ If } x \in [-C_i^{m-2},0)\\
	-C_i^{m-1} & \mbox{ If } x \in [-C_i^{m-2}+D_i^{m-2}-T_i, -C_i^{m-2})
   \end{cases}
\end{split}
\]
Meanwhile $\Delta_2(x)$ will first increases to $y_1=dbf(J_i^{*_B},S_m,\mathit e)|r(J_i^{*_B})+D_i^{m-1}=\mathit e$ (assuming at this time $x=x_1$), and then increases at most linearly to $C_i^{m-1}$, i.e., 
\[
	\begin{split}
	\Delta_2(x)
   \begin{cases}
	0 &\mbox{ If } x \in (x_1,0)\\
	y_1+(x_1-x)& \mbox{ If } x\in[-C_i^{m-1}+y_1+x_1, \leq x_1] \\
	C_i^{m-1}& \mbox{otherwise}
   \end{cases}
\end{split}
\]
Obviously if $x_1<-C_i^{m-2}$, then $\Delta_1(x)+\Delta_2(x)\leq 0$ and  $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)|L_i=m-1$ maximizes when $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}$. Else if $x_1 \geq -C_i^{m-2}$,  then as long as $x_1+y_1>0$,  $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)|L_i=m-1$  maximizes when $x=x_1$, i.e.,  $r(J_i^{*_A})=mod(\mathit e- D_i^{m-1},T_i)-T_i$. Otherwise $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)|L_i=m-1$ maximizes when $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}$.

In sum we can prove $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)|L_i=m-1$ maximizes when $r(J_i^{*_A})=-D_i^{m-2}+C_i^{m-2}$ or $r(J_i^{*_A})=mod(\mathit e- D_i^{m-1},T_i)-T_i$.  


\end{proof}



Task $\tau_i|_{L_i\geq m}$ generates maximum demand during $[S_{m-1}=0,\mathit e)$ if $r(J_i^{*_C})=mod(\mathit e- D_i^{m},T_i))-T_i$ (i.e, the last job release before $\mathit e$ has $d(J_i^L,m)=\mathit e$) or $r(J_i^{*_C})=mod(\mathit e- D_i^{m-1},T_i)-T_i$ (i.e., $d(J_i^L,m-1)=\mathit e$) or $r(J_i^{*_C})=-D_i^{m-2}+C_i^{m-2}$ and all the jobs are released as soon as possible with period $T_i$. 
\begin{proof}

If  ($\mathit e-S_m>D_i^m$): In this case $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)|L_i=m$ is maximized when $r(J_i^{*_C})=mod(\mathit e- D_i^{m},T_i))-T_i$. This is because that as $r(J_i^{*_C})$ increases, the demand of the last job released before $\mathit e$ $dbf(J_i^L,S_m,\mathit e)$ would decrease from $C_i^m$ to $0$ while the increase in demand of $J_i^{*_C}$ and $J_i^{*_D}$ (if exists) is bounded by $C_i^m$; On the other hand as $r(J_i^{*_C})$ decreases,  $dbf_{m}(J_i^{*_C},S_m,\mathit e)$ and $dbf_{m}(J_i^{*_D},S_m,\mathit e)$ may decrease while the demand of other jobs remain the same.


If ($\mathit e-S_m<D_i^m-D_i^{m-1}$): In this case, no job of $\tau_i$ could execute as much as $C_i^m$. Thus $\tau_i$ behaves as a task with $L_i=m-1$ and hence from Lemma~\ref{lem:pat2} we know $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)$ is maximized  when $r(J_i^{*_C})\in\{-D_i^{m-2}+C_i^{m-2}, mod(\mathit e- D_i^{m-1},T_i)-T_i\}$.

If  ($D_i^m-D_i^{m-1} \leq \mathit e-S_m\leq D_i^m$),  and initially set $r(J_i^{*_C})=mod(\mathit e- D_i^{m},T_i))-T_i$ (i.e., $d(J_i^{*_C},m)/d(J_i^{*_D},m)=\mathit e$), then at most one job (either $J_i^{*_C}$ or  $J_i^{*_D}$ ) could generate execution demand as much as $C_i^m$.  If at this time  $mod(\mathit e- D_i^{m},T_i))-T_i \geq -D_i^{m-2}+C_i^{m-2}$, then $dbf(J_i^{*_C})$ as well as $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)$ are already maximized.  

Otherwise if at this time,  $mod(\mathit e- D_i^{m},T_i))-T_i < -D_i^{m-2}+C_i^{m-2}$, as we shift the release pattern right, i.e.,  $r(J_i^{*_C})=mod(\mathit e- D_i^{m},T_i))-T_i+x|x>0$,   no job of $\tau_i$ would execute as much as $C_i^m$ and hence $\tau_i$ behaves like a task with $L_i=m-1$. Else if we shift the release pattern left, i.e.,  $r(J_i^{*_C})=mod(\mathit e- D_i^{m},T_i))-T_i+x|x<0$, both the execution demand of all jobs would decrease or stay the same, and hence the total execution demand would only decrease or remain the same. 

 
In sum  we can conclude that the total demand, $dbf^{\mbox{\tiny{2}}}_{m}(\tau_i,S_m,\mathit e)|L_i=m$ ,  is maximized if $r(J_i^{*_C})=-D_i^{m-2}+C_i^{m-2}$ or $r(J_i^{*_C})=mod(\mathit e- D_i^{m-1},T_i)-T_i$, or $r(J_i^{*_C})=mod(\mathit e- D_i^{m},T_i)-T_i$
\end{proof}

































